A general approximation lower bound in $L^p$ norm, with applications to feed-forward neural networks

We study the fundamental limits to the expressive power of neural networks. Given two sets $F$, $G$ of real-valued functions, we first prove a general lower bound on how well functions in $F$ can be approximated in $L^p(\mu)$ norm by functions in $G$, for any $p \geq 1$ and any probability measure $\mu$. The lower bound depends on the packing number of $F$, the range of $F$, and the fat-shattering dimension of $G$. We then instantiate this bound to the case where $G$ corresponds to a piecewise-polynomial feed-forward neural network, and describe in details the application to two sets $F$: H{\"o}lder balls and multivariate monotonic functions. Beside matching (known or new) upper bounds up to log factors, our lower bounds shed some light on the similarities or differences between approximation in $L^p$ norm or in sup norm, solving an open question by DeVore et al. (2021). Our proof strategy differs from the sup norm case and uses a key probability result of Mendelson (2002).

==> checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~1.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} We describe several possible extensions to our work in Section \ref{sec:Barron}. We also acknowledge, in the paragraph above Proposition 6, that extending Proposition 6 to other activation functions (such as ReLU) would be interesting and describe what we think is the main difficulty in Footnote~3. We also state several times that our lower bounds match the upper bounds up to a logarithmic factor, not exactly.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{} Our work is purely theoretical and we do not anticipate any  negative impact to it.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} The main notations and hypotheses are in Section 1. The functional spaces are defined at the beginning of the section concerning them. All the details concerning the networks architecture are always described in the theorems and propositions.
        \item Did you include complete proofs of all theoretical results? \answerYes{} The proof of the main result is in the article, Section \ref{main_result_proof}. The main corollary is proved in the supplement, Appendix~\ref{Appendix}. The proofs of the statements obtained when applying the main result are in the supplement. The proof of the upper bound described in Proposition 6 is also in the supplement.
\end{enumerate}


\item If you ran experiments... {\bf The article does not contain experiments.}
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...{\bf We do not use any existing asset.}
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...{\bf We did not use crowdsourcing nor conducted research with human subjects.}
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> oldlemma7.tex <==
\begin{lemma}\label{proprietes fct f}
We define $f(x) = \frac{x^{\alpha}}{\log^2(rPx)}$ for $x \geq 1$.
\begin{itemize}
    \item[i)] $f$ is increasing on $[\frac{2^{\frac{2}{\alpha}}}{r}, +\infty)$ and $\lim_{x\to +\infty} f(x) = +\infty$.
    \item[ii)] for all $b>0$, there exist $x_1$ such that , for all $x \geq x_1$ we have
    $$ b f(x) \geq f\left(\left(\frac{b}{2}\right)^{\frac{1}{\alpha}}x\right) .$$
\end{itemize}
    
\end{lemma}

\begin{proof}


\textbf{Proof of i):}
We have $$f'(x) = \frac{\alpha x^{\alpha-1} \log^2(rPx)-x^{\alpha}2 \log(rPx) \frac{1}{x}   }{\log^4(rPx)} = \frac{ x^{\alpha-1} \log(rPx)(\alpha \log(rPx)- 2   )}{\log^4(rPx)}$$
Hence, for $x > \frac{ 2^{\frac{2}{\alpha}} }{rP}$, $f'(x)>0$ and $f$ is increasing on $\left(\frac{ 2^{\frac{2}{\alpha}} }{rP}, +\infty\right)$. 
Since $P \geq 1$, $f$ is increasing on $[\frac{2^{\frac{2}{\alpha}}}{r} ,+\infty ) \subset \left(\frac{ 2^{\frac{2}{\alpha}} }{rP}, +\infty\right)$.

The limit at infinity is due to $\alpha>0$.

\textbf{Proof of ii):}
Let $a>0$. We have 
\begin{align*}
    \frac{f(ax)}{f(x)} = a^{\alpha} \frac{\log^{2}(rPx)}{\log^{2}(rPax)} \xrightarrow{x \to \infty} a^{\alpha}
\end{align*}
Therefore there exists $x_1>0$ such that for all $x \geq x_1$,
$\frac{f(ax)}{f(x)} \leq 2a^{\alpha}$. Hence, denoting by $b=2a^{\alpha}$, we obtain $b f(x) \geq f\left(\left(\frac{b}{2}\right)^{\frac{1}{\alpha}}x\right)$.
\end{proof}

==> oldproofthm.tex <==
\begin{proof}[Proof (of Theorem \ref{main_result})]
\label{main_result_proof}
First, observe that Assumption (\ref{packing_lower_bound}) along with Lemma \ref{lemma_FS_0_pack_0} entail $\fat_{\frac{\varepsilon}{32}}(G) \geq 1$. Let $E := \sup_{f \in F} \inf_{g \in G} \|f - g\|_{L^p(\mu)}$ denotes the $L^p(\mu)$ approximation error of $F$ by $G$. In the following, we prove that for any $\varepsilon > E$, we must have $\varepsilon \geq \min\{\varepsilon_1, c_2 P^{-\frac{1}{\alpha}} \log^{-\frac{2}{\alpha}}(P)\}$. We will then conclude by letting $\varepsilon$ tend to $E$. To this end, we eventually want to apply Proposition \ref{result_mendelson} to $G$. However, functions in $G$ are not necessarily bounded and the proposition does not automatically apply. To work around this issue, we define for any function $g$ in $G$ its truncature to $[a,b]$ as the function $\tilde{g}$ given for all $x \in \mathcal{X}$ by $\tilde{g}(x) = \min(\max(a,g(x)), b)$, and we consider the associated set
$$
G_{[a,b]} = \left\{ \tilde{g}, g \in G \right\}.
$$

\noindent Functions in $G_{[a,b]}$ thus have values in $[a,b]$ which is the same range as $F$.


%Moreover, Lemma \ref{lemma_fatG} yields that the $\gamma$-fat-shattering dimension of $G_{[a,b]}$ is less than that of $G$ for any $\gamma > 0$.

%Now let $\varepsilon > E$.
Let $\varepsilon_1' = \min(\frac{\varepsilon_0}{3},2)$. If $E \geq \varepsilon_1'$, \eqref{main_result_equation} trivially holds. We assume in the sequel that $E < \varepsilon_1'$, and consider $\varepsilon$ such that $\varepsilon_1' > \varepsilon > E$.
Because functions in $F$ have values in $[a,b]$, Lemma$~$\ref{lemma_supinf_G} in Appendix \ref{Appendix} yields that for any probability measure $\mu$, the $L^p(\mu)$ approximation error of $F$ by $G_{[a,b]}$ is less than that of $F$ by $G$. We thus have $\sup_{f \in F} \inf_{g \in G_{[a,b]}} \|f - g\|_{L^p(\mu)} < \varepsilon$. Hence, since $\varepsilon \leq \varepsilon_0/3$, Lemma$~$\ref{lemma_entropy_G_vs_F} along with (\ref{packing_lower_bound}) entail
\begin{align}
    \label{metric_entropy_G_ab}
    \log M\left(\varepsilon, G_{[a,b]}, \|\cdot\|_{L^p(\mu)}\right) \geq \log M\left(3\varepsilon, F, \|\cdot\|_{L^p(\mu)}\right) \geq c_0 (3\varepsilon)^{-\alpha}.
\end{align}

\noindent Note that this implies in particular that $\fat_{\frac{\varepsilon}{32}}(G_{[a,b]}) \geq 1$, by (\ref{equation_mendelson}). Moreover, because $G$ has finite pseudo dimension, it also has finite $\gamma$-fat-shattering dimension for all $\gamma > 0$. Lemma \ref{lemma_fatG} in Appendix \ref{Appendix} thus entails that $G_{[a,b]}$ has finite $\gamma$-fat-shattering dimension for all $\gamma > 0$. Proposition $1$ thus applies to $G_{[a,b]}$ and yields, when combined with (\ref{metric_entropy_G_ab}),
\begin{align}
    \label{mendelson_vs_epsilon}
    c_0(3\varepsilon)^{-\alpha} \leq
    c \fat_{\frac{\varepsilon}{32}}(G_{[a,b]}) \log^2 \left(\frac{2(b-a) \fat_{\frac{\varepsilon}{32}}(G_{[a,b]})}{\varepsilon}\right),
\end{align}

\noinent for some $c > 0$ depending only on $p$ (\textcolor{red}{A verifier qd mm dans sa preuve si c'est que p}). Now simple calculations show that the function $t \mapsto c t \log^2 \left( \frac{2t}{\varepsilon} \right)$ is non-decreasing on $[\varepsilon/2,+\infty)$.  

Since $\varepsilon \leq 2$ and $\fat_{\frac{\varepsilon}{32}}(G_{[a,b]}) \geq 1$, using Lemma \ref{lemma_fatG} in Appendix \ref{Appendix}, we obtain
\begin{align*}
    \frac{\varepsilon}{2} \leq \fat_{\frac{\varepsilon}{32}}(G_{[a,b]}) \leq \fat_{\frac{\varepsilon}{32}}(G) \leq \Pdim(G)
\end{align*}
Therefore, 
\begin{align}
    c_0(3\varepsilon)^{-\alpha} \leq
    c \Pdim(G) \log^2 \left(\frac{2(b-a) \Pdim(G)}{\varepsilon}\right).
\end{align}


%Hence, since $\fat_{\frac{\varepsilon}{32}}(G_{[a,b]}) \geq 1$, it suffices to take $\varepsilon < 1$ so that one can only increase the right-hand side of (\ref{mendelson_vs_epsilon}) by taking $t > \fat_{\frac{\varepsilon}{32}}(G)$. Therefore, since $\fat_{\gamma}(G_{[a,b]}) \leq \fat_{\gamma}(G)$ by Lemma \ref{lemma_fatG}, and since for any $\gamma > 0$, $\fat_\gamma(G) \leq \Pdim(G)$, one can replace $\fat_{\frac{\varepsilon}{32}}(G_{[a,b]})$ with $P := \Pdim(G)$ in (\ref{mendelson_vs_epsilon}).
Solving this inequation in $\varepsilon$ (refer to Appendix \ref{function_study} for details), we get
\begin{align}
    \label{main_result_proof_conclusion}
    %\varepsilon \geq c_2 P^{-\frac{1}{\alpha}} \log^{-\frac{2}{\alpha}}(P),
    \varepsilon \geq \min\left\{\varepsilon_1'', \ c P^{-\frac{1}{\alpha}} \log^{-\frac{2}{\alpha}}P\right\},
\end{align}

\noindent for some constants $c$, $\varepsilon_1'' > 0$ depending on $d$ and $p$.
%whenever $\varepsilon \leq \varepsilon_0'$ for some constant $\varepsilon_0' > 0$, and setting $P := \Pdim(G)$ for brevity. It remains to set $\varepsilon_1 := \min\{\varepsilon_0/3, \varepsilon_0'\}$ to obtain $\varepsilon \geq \min\left\{\varepsilon_1, \ c_7 P^{-\frac{1}{\alpha}} \log^{-\frac{2}{\alpha}}P)\right\}$.
Taking $\varepsilon_1 = \min(\varepsilon'_1, \varepsilon''_1)$ concludes the proof. 
\end{proof}

==> oldsection2.tex <==
\subsection{Main result}


Our generic lower bound reads as follows, and is proved in \textcolor{red}{Section \ref{main_result_proof}}.
%In this subsection, we get rid of the above assumption and generalize the result by assuming the lower bound is $a(\varepsilon)$.

\begin{theorem}
\label{general_thm}
Let $F$ and $G$ be two sets of functions defined on a domain $\mathcal{X} \subset \mathbb{R}^d$ endowed with a probability measure $\mu$, where functions in $F$ are valued in a finite range $[a,b]$. Assume there exists $\varepsilon_0 >0$ such that for any $\varepsilon \leq \varepsilon_0$
$$
\log M\left(\varepsilon, F, \|\cdot\|_{L^p(\mu)}\right) \geq a(\varepsilon) \quad \text{ and } \quad \fat_{{\varepsilon}}(G) \leq b(\varepsilon).
$$

Therefore, there exists a constant $c$ depending only on $p$ such that
\begin{align}
    \label{lower bound thm general}
    \sup_{f \in F} \inf_{g \in G} \|f - g\|_{L^p(\mu)} \geq \min\left(\varepsilon_0\textcolor{red}{/3}, \inf\left\{\varepsilon: a(\varepsilon) \leq c b\left(\frac{\varepsilon}{32}\right) \log^2\left(\frac{2 b\left(\frac{\varepsilon}{32}\right)}{\varepsilon}\right)\right\} \right) .
\end{align}
\end{theorem}

% \begin{remark}
% Sometimes we can have a direct upper bound on the covering number of the approximating space $G$ (e.g., Quantized Networks). In this case we do not need to include any notion of fat-dimension and the bound is obtained just by using Lemma \ref{lemma_entropy_G_vs_F} and solving for $\varepsilon$.
% \end{remark}

By assuming a finite pseudo-dimension of $G$, and that the logarithm of the packing number of the space function $F$ grows at least polynomially in $1/\varepsilon$, which is the case for many examples of interest (see the next sections), one can obtain a closed-form for the lower bound.
An important special case is when the approximation set $G$ is  the set $H_{\mathcal{A}}$ of all functions that can be implemented by tuning the weights of a feed-forward neural network with architecture $\mathcal{A}$.
By combining Theorem \ref{main_result} with known bounds on the pseudo-dimension \cite{pmlr-v65-harvey17a}, we can obtain bounds with respect to the number of weights and layers.
This is the statement of the next corollary, which is proved in Section \ref{main_result_proof}.


%\textcolor{red}{Est-ce qu'on énoncerait pas le résultat pour $\fat_{\gamma}(G) < \infty$, plutôt que $\Pdim(G) < \infty$ (car ça doit encore fonctionner) ? $\rightarrow$ voir ce que ça changerait dans le raisonnement dans l'appendix}



\begin{coro}
\label{main_result}
%Let $F$ be a set of functions from $\mathcal{X} \subset \mathbb{R}^d$ to $[a,b] \subset \mathbb{R}$, where the non-empty measurable set $\mathcal{X}$ is endowed with probability measure $\mu$. Assume there exist $\alpha,c_0,\varepsilon_0 >0$ such that for any $\varepsilon \leq \varepsilon_0$

% \begin{align}
% \label{packing_lower_bound}
%     \log M\left(\varepsilon, F, \|\cdot\|_{L^p(\mu)}\right) \geq c_0 \varepsilon^{-\alpha}.
% \end{align}


% Let $G$ be a set of functions from $\mathcal{X}$ to $\mathbb{R}$ with non-zero, finite pseudo dimension $P = \Pdim(G)$. Then, there exist $\varepsilon_1 > 0$ and a constant $c_1 > 0$ depending only on $p,d$ and $\alpha$ such that

Under the same assumptions of Theorem \ref{general_thm}, and assuming in addition that $P:=\Pdim(G) < +\infty$ and that $a(\varepsilon) = c_0 \varepsilon^{-\alpha}$ for constants $c_0,\alpha>0$, the lower bound \eqref{lower bound thm general} reads:
\begin{align}
    \label{main_result_equation}
    \sup_{f \in F} \inf_{g \in G} \|f - g\|_{L^p(\mu)} \geq \min\left\{\varepsilon_1, \ c_1 P^{-\frac{1}{\alpha}}\log^{-\frac{2}{\alpha}}(P)\right\} .
\end{align}

In particular, if $G$ is the set of all functions that can be represented by a feed-forward neural network with a fixed architecture of depth $L \geq 1$, $W \geq 1$ variable weights, and a piecewise-polynomial activation function of maximal degree $\nu \in \mathbb{N}$, then \eqref{main_result_equation} reads
\begin{align}
    \sup_{f \in F} \inf_{g \in {H}_\mathcal{A}} \|f - g\|_{L^p(\mu)} \geq
    \left\{
    \begin{array}{l l}
         c_1  W^{-\frac{2}{\alpha}} \log^{-\frac{2}{\alpha}}(W) & \text{ if } \nu \geq 2, \\
         c_2  (LW)^{-\frac{1}{\alpha}} \log^{-\frac{3}{\alpha}}(W)& \text{ if } \nu=1, \\
         c_3  W^{-\frac{1}{\alpha}} \log^{-\frac{3}{\alpha}}(W)& \text{ if } \nu=0 .
    \end{array}
    \right.
\end{align}
where $c_1,c_2,c_3>0$ are constants that only depend on $d$, $p$ and $\alpha$.
\end{coro}

\textcolor{red}{El Mehdi: J'ai viré (commenté sur le latex) la remarque pour quand la metric entropy est lower bounded par $\varepsilon^{-\alpha}\log^\beta\left(1/\varepsilon\right)$. A voir si on la remet ou pas.}
% \begin{remark}
% Though Assumption \eqref{packing_lower_bound} covers many examples of interest such as Hölder space, monotonic functions space and Barron space (see the next sections), the above theorem can be generalized.
% As shown in Theorem \ref{general_thm}, at the end of Section \ref{sec: general approximation lower bound}, when replacing \eqref{packing_lower_bound} by a general lower bound on the log packing number, one can obtain a more general form of the lower bound. In particular, under the assumption that $\log M\left(\varepsilon, F, \|\cdot\|_{L^p(\mu)}\right) \geq c_0 \varepsilon^{-\alpha}\log^\beta\left(1/\varepsilon\right)$, $\beta \geq 0$, the right-hand side of \emph{(\ref{main_result_equation})} becomes $\min\left\{\varepsilon_1, \ c_1 P^{-\frac{1}{\alpha}}\log^{\frac{\beta - 2}{\alpha}}(P)\right\}$.
% \end{remark}





% \begin{coro}
% \label{main_corollary}
% Let $F$ be a set of functions from $\mathcal{X} \subset \mathbb{R}^d$ to $[a,b] \subset \mathbb{R}$, where the non-empty measurable set $\mathcal{X}$ is endowed with probability measure $\mu$. Assume there exist $\alpha,c_0,\varepsilon_0 >0$ such that for any $\varepsilon \leq \varepsilon_0$,

% \begin{align}
% %\label{packing_lower_bound}
%     \log M\left(\varepsilon, F, \|\cdot\|_{L^p(\mu)}\right) \geq c_0 \varepsilon^{-\alpha}.
% \end{align}


% Let $\sigma : \mathbb{R} \rightarrow \mathbb{R}$ be a piecewise-polynomial function having maximal degree $\nu \in \mathbb{N}$.
% Let $H_{\mathcal{A}}$ be the set of functions implemented by a neural network with an architecture $\mathcal{A}$ with activation $\sigma$, $W$ weights and $L$ layers.
% Then, there exist constants $c_1,c_2,c_3,W_{\emph{min}}>0$ depending only on $p,d$ and $\alpha$ such that for all $W \geq W_{\emph{min}}$,
% \begin{align}
%     \sup_{f \in F} \inf_{g \in {H}_\mathcal{A}} \|f - g\|_{L^p(\mu)} \geq
%     \left\{
%     \begin{array}{l l}
%          c_1  W^{-\frac{2}{\alpha}} \log^{-\frac{2}{\alpha}}(W) & \text{ if } \nu \geq 2, \\
%          c_2  (LW)^{-\frac{1}{\alpha}} \log^{-\frac{3}{\alpha}}(W)& \text{ if } \nu=1, \\
%          c_3  W^{-\frac{1}{\alpha}} \log^{-\frac{3}{\alpha}}(W)& \text{ if } \nu=0 .
%     \end{array}
%     \right.
% \end{align}
% \end{coro}



% \textcolor{red}{Clarifier la remarque ci-dessous et la raccourcir}

% \begin{remark}
% It is worth noting that \emph{(\ref{main_result_equation})} can be reversed to obtain a lower bound on $\Pdim(G)$, and then combined with upper  bounds on $\Pdim(G)$ to produce new estimates in terms of the approximation error. This applies for instance in the context of neural network approximation, where this allows bound from below the minimal number of weights required to achieve a certain approximation error \textcolor{red}{citer un exemple}.
% \end{remark}


% \begin{remark}
% Our result provides an answer to an open problem raised by DeVore et al. in \cite{devore_hanin_petrova_2021} about the difficulty of obtaining $L^p$ approximation lower bounds for $1 \leq p < +\infty$. After showing an upper bound for the $L^\infty$ approximation error of unit balls in Besov spaces by neural networks (Theorem $8.12$), the authors make the following comment : ``\emph{When we move to the case $p < +\infty$, the situation is even less clear. First, Theorem $8.12$ does give a super rate. However, we have no corresponding lower bounds that come close to matching this rate because we cannot use the VC dimension theory for $L^p$ approximation. In summary, for all Besov spaces that compactly embed into $L^p (\Omega)$, we obtain error bounds for approximation in $L^p (\Omega)$ strictly better than classical methods. What is missing vis-à-vis Problem $8.13$ is what the best bounds are and how we prove lower bounds for approximation rates in $L^p (\Omega)$, $p \neq  \infty$''.}
% \end{remark}

==> oldstuff-Barron.tex <==
\subsection{\red{Old stuff}}

\subsubsection{The definition of Barron functions}
\label{sec:barron_space_def}


\subsubsection{Proof of Proposition \ref{prop_lb_barron}}
\label{sec:proof_barron_lb}


\subsubsection{Extension of the upper bound from \cite{Barron} to ReLU neural networks}
\label{appendix_barron_UB_extension}

In this subsection, we first recall the upper bound for the approximation of Barron functions by sigmoidal neural networks in $L^2(\mu)$ norm. Then we prove that the result still holds for ReLU neural networks, as stated in Proposition \ref{prop_upper_bound_barron_space}.

\begin{prop}
    \label{prop_barron_original}
    Let $d \in \NN^*$. For any integer $W \geq 1$, there exists a sigmoidal activation feed-forward neural network architecture $\mathcal{A}$ with one hidden layer and $W$ weights such that, for any probability measure $\mu$ over $[-1,1]^d$,

\begin{equation}
    \label{equation_borne_sup_barron} \sup_{f \in F^B_{d}}\inf_{g \in H_{\mathcal{A}}} \|f - g\|_{L^2(\mu)} \leq 
    c_1 W^{-1/2},
\end{equation}

\noindent where $c_1 := (2 \sqrt{d} B)^2$.
\end{prop}

Now we prove that the result still holds, up to a factor $\sqrt{2}$, when replacing the sigmoidal activation by the ReLU activation. This is a direct consequence of the following lemma :

\begin{lemma}[\cite{JMLR:v20:17-612}]
    \label{lemma_relu_sigmoidal}
    Denote by $\sigma$ the ReLU function $\sigma : x \mapsto \max\{0,x\}$. The function $\sigma' : x \mapsto \sigma(x) - \sigma(x-1)$ is a sigmoidal function. Moreover, any one-hidden-layer feed-forward network with activation $\sigma'$ and $W$ weights can be expressed as a one-hidden-layer feed-forward network with the ReLU activation and $2W$ parameters.
\end{lemma}

\begin{proof}
    The fact that $\sigma'$ is a sigmoidal function is straightforward. For the second fact, notice that a function $g$ over $\mathbb{R}^d$ implemented by a feed-forward network with one hidden layer, $W$ weights, $n$ units and activation $\sigma'$ reads as
    $$
    g(x) = \sum_{i=1}^n c_i \sigma'\left(\langle a_i, x \rangle + b_i\right),
    $$
    for some parameters $c_i \in \mathbb{R}$, $a_i \in \mathbb{R}^d$ and $b_i \in \mathbb{R}$. The total number of non-zero entries in the vectors $a_i$ being smaller than $W$. It thus holds that
    $$
    g(x) = \sum_{i=1}^{2n} c_i \sigma\left( \langle a_i,x \rangle + b_i \right),
    $$
    where for $i = 1, \ldots, n$, $c_{i+n} = -c_i$, $a_{i+n} = a_i$ and $b_{i+n} = b_i - 1$. This is a one-hidden-layer feed-forward network with the ReLU activation and $2W$ parameters.
\end{proof}

\subsection{Proof of Proposition \ref{prop_metric_entropy_barron}}
\label{appendix_barron_proof_metric_entropy}

\textcolor{red}{In progress}

The outline of the proof is as follows. First, we introduced a set of functions defined in \cite{8006754}, that the authors prove to have $\varepsilon$-packing number at least $c\varepsilon^{-2}$, for some constant $c$ independent from $\varepsilon$. Then we notice that the functions in this set can be approached arbitrarily close in $L^2$ distance by functions in the Barron space, and we conclude using Lemma \ref{lemma_entropy_G_vs_F}.

The following lemma introduces the functions set from \cite{8006754} and is proved in the first part of the proof of their Theorem $1$.

\begin{lemma}
    \label{lemma_F_0_Klusowsky_Barron}
    Let $d \in \NN^*$, $B>0$. Let $\varepsilon > 0$ and let $v_0 > \max\{3,d\}$ be such that $\varepsilon \geq B/(\sqrt{2}(v_0 + d)(1+v_0/d)^{d/4})$. Let $\Lambda = \{\theta \in \mathbb{Z}^d \ : \ \|\theta\|_1 \leq v_0 \}$, and let $M = |\Lambda|$, $L \leq M/10$, $B' = \frac{B}{\sqrt{2}(v_0 + d)}$. Let $\mathcal{S} = \left\{  \sigma \in \{0,1\}^M \ : \ \|\sigma\|_1 = L \right\}$.
    Define
    $$
    \mathcal{F}_0 = \left\{ f_{\sigma}(x) = \frac{B'}{L} \sum_{k=1}^M \sigma_k \sqrt{2} \sin( \theta_k \cdot x), \ x \in [-1,1]^d \ : \ \sigma \in \mathcal{S} \right\},
    $$
    for some enumeration $\theta_1, \ldots, \theta_M$ of $\Lambda$. Denoting by $\mu$ the uniform probability over $[-1,1]^d$, there exists constants $c, \varepsilon_0 > 0$ depending only on $d$ and $B$ such that for any $0 < \varepsilon \leq \varepsilon_0$, $\log M\left(\varepsilon, \mathcal{F}_0, \|\cdot\|_{L^2(\mu)}\right) \geq c \varepsilon^{-2}$.
\end{lemma}

The functions in the set $\mathcal{F}_0$ are not in the Barron space because these are weighted sums of sine functions$~$; as such, any $f \in \mathcal{F}_0$ writes as $f(x) = \int_{\mathbb{R}^d} e^{i \omega \cdot x} \hat{f}(\dd \omega)$, where $\hat{f}$ is a weighted sum of Dirac measures. We aim to approximate $f$ with a sequence of functions $(f_n)_{n \geq 1} \subset F^{B}_{d}$ that has Fourier representation $f_n(x) = \int_{\mathbb{R}^d} e^{i \omega\cdot x} \hat{f}_n(\omega) \dd \omega$ with $\hat{f}_n(\dd \omega) = \hat{f}_n(\omega) \dd \omega$ close to a Dirac measure while being continuous, and such that $\int_{\mathbb{R}^d} \|\omega\|_2 |\hat{f}_n(\omega)| \dd \omega < +\infty$.


\begin{proof}[Proof (of Proposition \ref{prop_metric_entropy_barron}).]
In what follows, we reuse the notations introduced in Lemma \ref{lemma_F_0_Klusowsky_Barron}. We consider the set of functions
$$
\mathcal{F}_{1,\varepsilon} = \left\{f_{\sigma,\varepsilon}(x) = \frac{B'}{L} \sum_{k=1}^M \sigma_k \sqrt{2} \sin \left( \theta_k \cdot x\right) \prod_{j=1}^d \frac{\sin( x_j \sqrt{\varepsilon'})}{x_j \sqrt{\varepsilon'}}, \ x \in [-1,1]^d \ : \ \sigma \in \mathcal{S} \right\},
$$
where we have set $\varepsilon' := \varepsilon/(2^d \sqrt{2}B')$.
We prove that $\mathcal{F}_1$ approximates $\mathcal{F}_0$ with error $\varepsilon$ in $L^2(\mu)$ norm (like in Lemma \ref{lemma_F_0_Klusowsky_Barron}, $\mu$ denotes the uniform probability measure over $[-1,1]^d$).

We have for all $y \in [-1,1]$

\begin{align*}
     \frac{\sin(y)}{y} \leq 1+\frac{y^2}{3}
\end{align*}
Hence using it for $y = x \sqrt{\varepsilon'}$, where $x \in [-1,1]$ and $\varepsilon' \in (0,1)$ we obtain
\begin{align*}
     \frac{\sin(x \sqrt{\varepsilon'})}{x \sqrt{\varepsilon'}} \leq 1+{x^2 \sqrt{\varepsilon'}^2} \leq 1 + {\varepsilon'}  
\end{align*}
Hence, we have 
\begin{align*}
    \prod_{j=1}^d \frac{\sin( x_j \sqrt{\varepsilon'})}{x_j \sqrt{\varepsilon'}} - 1 \leq (1+{\varepsilon'})^d - 1 \leq 2^d \varepsilon'
\end{align*}
therefore
\begin{align*}
    \|f_0 - f_1 \|_{L^2(\mu)}
    &\leq \|f_0 - f_1 \|_{\infty} \\
    &\leq \frac{B'}{L} \sum_{k=1}^M \sigma_k \sqrt{2} \left\| \sin \left( \theta_k \cdot x\right) \right\|_{\infty} \left\|\prod_{j=1}^d \frac{\sin( x_j \sqrt{\varepsilon'})}{
    x_j \sqrt{\varepsilon'}} - 1 \right\|_\infty \\ 
    & \leq 2^d \sqrt{2} \frac{B'}{L} L \varepsilon' \\
    \|f_0 - f_1\|_{L^2(\mu)}
    &\leq \varepsilon,
\end{align*}

where in the second line, we used the fact that $\sigma_k$ is equal to $0$ on all but $L$ coordinates. Now we prove that functions in $F_1$ are in the Barron space.

We denote by $g_k$ the function over $[-1,1]^d$ defined by
\begin{align*}
    g_{k}(x) = \sin \left( \theta_k \cdot x\right) \prod_{j=1}^d \frac{\sin( x_j \sqrt{\varepsilon})}{x_j \sqrt{\varepsilon}},
\end{align*}

One can easily check that
\begin{align*}
    g_{k}(x) = \int_{\mathbb{R}^d} e^{i \omega \cdot x} \hat{g}_{k}( \omega) \dd \omega
\end{align*}
where
\begin{align*}
     \hat{g}_{k}(\omega) =  \frac{1}{2^d 2i \sqrt{\varepsilon}} \left(\mathds{1}_{\Delta(\theta_k)}(\omega) - \mathds{1}_{\Delta(-\theta_k)}(\omega)\right)
\end{align*}

Let us show that $\mathcal{F}_{1,\varepsilon}$ is a subset of $F^{B}_{d}$ for all $n \geq 1$. First, by writing $\hat{f}_{\sigma,n}(\omega) := \frac{B'}{L} \sum_{k=1}^M \sigma_k \sqrt{2} \hat{g}_{k}(\omega)$, it is clear that $f_{\sigma, n}$ admits a Fourier representation as in (\ref{fourier_representation}). It remains to prove that $\int_{\mathbb{R}^d} \|\omega\|_2 |\hat{f}_{n}(\omega)| \leq B$. Given the expression of $\hat{f}_{\sigma, n}$ and that of $\hat{g}_{n,k}$, and bounding from above the norm $\|\cdot\|_2$ by the norm $\|\cdot\|_1$, we have that
\begin{align*}
    \int_{\mathbb{R}^d} \|\omega\|_2 |\hat{f}_{\sigma,n}(\omega)| \dd \omega
    &\leq \frac{\sqrt{2}B'}{L} \sum_{k=1}^M \sigma_k \int_{\Delta_n(\theta_k) \cup \Delta_n(-\theta_k)} \|\omega\|_1 \frac{(n/2)^d}{2} \dd \omega,
\end{align*}
Now, because $\|\theta_k\|_1 \leq v_0$ for all $k$, and by definition of $\Delta_n(\theta_k)$, we have that $\|\omega\|_1 \leq v_0 + d$ for any $\omega \in \Delta_n(\theta_k) \cup \Delta_n(-\theta_k)$, $n \geq 1$. Using the fact that $\Delta_n(\theta_k) \cup \Delta_n(-\theta_k)$ has Lebesgue measure at most $2(n/2)^{-d}$, and since $\sigma_k = 0$ on all but $L$ index $k$, we have that
\begin{align*}
    \int_{\mathbb{R^d}} \|\omega\|_2 |\hat{f}_{\sigma,n}(\omega)| \dd \omega
    &\leq \frac{\sqrt{2}B'}{L} L (v_0 + d) = B,
\end{align*}
which proves that $\mathcal{F}_{1,n} \subset F^B_{d}$.

\end{proof}




\begin{proof}[Proof (of Proposition \ref{prop_metric_entropy_barron}).]

 For $n \geq 1$, $\theta_k \in \Lambda$, we define
$$
\hat{g}_{n,k}(\dd \omega) = \hat{g}_{n,k}(\omega) \dd \omega =  \frac{(n/2)^d}{2i} \left(\mathds{1}_{\Delta_n(\theta_k)}(\omega) - \mathds{1}_{\Delta_n(-\theta_k)}(\omega)\right) \dd \omega,
$$
\noindent where $\Delta_n(\theta_k)$ is the cube of side-length $2/n$ centered at $\theta_k$. Denoting by $g_{n,k}$ the inverse-Fourier transform of $\hat{g}_{n,k}$, we have that $g_{n,k}(x) = \int_{\mathbb{R}^d} e^{i \omega \cdot x} \hat{g}_{n,k}(\dd \omega)$, which entails
\begin{align*}
    g_{n,k}(x)
    &=
    \frac{(n/2)^d}{2i}\left(\prod_{j=1}^d\left[\frac{e^{i \omega_j x_j}}{i x_j}\right]_{\theta_{kj} - 1/n}^{\theta_{kj} + 1/n} - \prod_{j=1}^d\left[\frac{e^{i \omega_j x_j}}{i x_j}\right]_{-\theta_{kj} - 1/n}^{-\theta_{kj} + 1/n}\right) \\
    &= \frac{(n/2)^d}{2i} \left( e^{i \theta_k \cdot x} - e^{-i \theta_k \cdot x} \right) \prod_{j=1}^d \left[ \frac{1}{i x_j} \left( e^{\frac{i x_j}{n}} - e^{-\frac{i x_j}{n}} \right) \right] \\
    &= \sin \left( \theta_k \cdot x\right) \prod_{j=1}^d \frac{\sin( x_j / n)}{x_j / n},
\end{align*}
\noindent where at the third line we used the Euler formula $e^{i t} - e^{-i t} = 2i \sin(t)$. Now similarly to $\mathcal{F}_0$, we set
$$
\mathcal{F}_{1,n} = \left\{f_{\sigma,n}(x) = \frac{B'}{L} \sum_{k=1}^M \sigma_k \sqrt{2} g_{n,k}(x), \ x \in [-1,1]^d \ : \ \sigma \in \mathcal{S} \right\}.
$$
Let us show that $\mathcal{F}_{1,n}$ is a subset of $F^{B}_{d}$ for all $n \geq 1$. First, by writing $\hat{f}_{\sigma,n}(\omega) := \frac{B'}{L} \sum_{k=1}^M \sigma_k \sqrt{2} \hat{g}_{n,k}(\omega)$, it is clear that $f_{\sigma, n}$ admits a Fourier representation as in (\ref{fourier_representation}). It remains to prove that $\int_{\mathbb{R}^d} \|\omega\|_2 |\hat{f}_{n}(\omega)| \leq B$. Given the expression of $\hat{f}_{\sigma, n}$ and that of $\hat{g}_{n,k}$, and bounding from above the norm $\|\cdot\|_2$ by the norm $\|\cdot\|_1$, we have that
\begin{align*}
    \int_{\mathbb{R}^d} \|\omega\|_2 |\hat{f}_{\sigma,n}(\omega)| \dd \omega
    &\leq \frac{\sqrt{2}B'}{L} \sum_{k=1}^M \sigma_k \int_{\Delta_n(\theta_k) \cup \Delta_n(-\theta_k)} \|\omega\|_1 \frac{(n/2)^d}{2} \dd \omega,
\end{align*}
Now, because $\|\theta_k\|_1 \leq v_0$ for all $k$, and by definition of $\Delta_n(\theta_k)$, we have that $\|\omega\|_1 \leq v_0 + d$ for any $\omega \in \Delta_n(\theta_k) \cup \Delta_n(-\theta_k)$, $n \geq 1$. Using the fact that $\Delta_n(\theta_k) \cup \Delta_n(-\theta_k)$ has Lebesgue measure at most $2(n/2)^{-d}$, and since $\sigma_k = 0$ on all but $L$ index $k$, we have that
\begin{align*}
    \int_{\mathbb{R^d}} \|\omega\|_2 |\hat{f}_{\sigma,n}(\omega)| \dd \omega
    &\leq \frac{\sqrt{2}B'}{L} L (v_0 + d) = B,
\end{align*}
which proves that $\mathcal{F}_{1,n} \subset F^B_{d}$.

Now, we prove that for any $\sigma \in \mathcal{S}$, $f_{\sigma,n}$ uniformly converges to $f_\sigma$. Note that this is true if and only if $\sup_{x \in [-1,1]^d}|g_{n,k}(x) - \sin(\theta_k \cdot x)|$ converges to $0$ as $n$ goes to $\infty$ for $k = 1, \ldots, M$. For any $x \in [-1,1]^d$, we have
\begin{align*}
    |g_{n,k}(x) - \sin( \theta_k \cdot x)|
    &= |\sin(\theta_k \cdot x)| \left|\prod_{j=1}^d \frac{\sin(x_j/n)}{ x_j /n} - 1\right| \\
    &\leq \left|\prod_{j=1}^d \left(1 + o(x_j /n)\right) - 1 \right| \\
    &\leq o(1/n),
\end{align*}
\noindent where in the second line we used the sine's Taylor expansion. We thus have $\lim\limits_{n \rightarrow \infty} \sup_{x \in [-1,1]^d} |g_{n,k}(x) - \sin(\theta_k \cdot x)| = 0$. Hence, since $\mathcal{F}_{1,n} \subset F^{B}_{d}$ for all $n \geq 1$, then for any $\varepsilon > 0$, $F^{B}_{d}$ approximates $\mathcal{F}_0$ in sup norm with error less than $\varepsilon$. The result follows from Lemma$~$\ref{lemma_entropy_G_vs_F}.
\end{proof}
